Fusion: A Framework for Unified Sequential Token AdaptatIon in VisiOn TraNsformers

Vision Transformers achieve strong image classification accuracy but process all image regions with nearly the same computation, even when many regions are redundant or uninformative. Recent adaptive inference methods reduce this cost by selectively compressing tokens or terminating inference early, but combining these mechanisms often causes unstable intermediate representations and accuracy degradation. We introduce Fusion, a unified adaptive inference framework that coordinates token merging, early exiting, and token pruning through a simple staged design: tokens are merged first, confidence is evaluated next, and pruning is applied only to samples that continue inference. This ordering allows the three mechanisms to operate cooperatively rather than competitively. Fusion further includes lightweight routing modules that adapt compression strength to each input and support inference-time adjustment of the accuracy--latency trade-off without retraining. On ImageNet-1k with DeiT-S, Fusion matches or surpasses state-of-the-art adaptive ViT methods at comparable compute budgets while reducing calibration error by up to $4\times$ and inference energy by $48\%$. Experiments across ImageNet-100, CIFAR-100, and ImageNette with multiple ViT backbones demonstrate consistent transferability without dataset-specific tuning.

==> sections/00_abstract.tex <==
\begin{abstract}
We present \modtp{}, a framework for combining token merging, early
exit, and token pruning into a single dynamic Vision Transformer.
Existing methods study these mechanisms separately; naively combining
them causes structural interference that costs accuracy. \modtp{}
eliminates this through three coordinated components: a sequential
composition protocol that orders the mechanisms, inline merge routers
that predict per-image and per-block merge ratios from the class
token, and profile-aware multiplicative scaling that shifts a single
trained checkpoint across operating points at inference time. The
framework is backbone-agnostic and applies to any plain ViT-family
transformer parameterised by embedding dimension $d$ and depth $L$.
On ImageNet-1k DeiT-S, \modtp{} matches the DynamicViT, EViT, and ToMe
operating points from a single trained checkpoint within $\pm 0.05$
percentage points (pp) of accuracy, achieves roughly $4\times$ better
expected calibration error than these baselines, and reduces energy
by $48\%$ at its power-save profile. Cross-dataset experiments on
ImageNet-100, CIFAR-100, and ImageNette with DeiT-S and ViT-Tiny
backbones confirm the recipe transfers without per-dataset tuning.
\end{abstract}


==> sections/01_introduction.tex <==
\section{Introduction}
\label{sec:intro}

Vision Transformers~\citep{dosovitskiy2021vit,touvron2021deit} dominate
image classification but spend the same compute on every input: a
$224\!\times\!224$ ViT processes 196 patch tokens through all twelve
transformer blocks, whether the input is a single object on a uniform
background or a cluttered street scene. Three independent lines of work
address this by reducing computation along different axes. Token pruning
drops uninformative tokens between
blocks~\citep{rao2021dynamicvit,liang2022evit}; token
merging~\citep{bolya2023tome} averages similar tokens; and early
exit~\citep{yin2022avit,xu2023lgvit,teerapittayanon2016branchynet} skips
late blocks on samples an intermediate classifier already finds easy.
Each of these mechanisms is studied in isolation and treats the ViT
backbone as a fixed substrate.

Combining all three in a single network is not straightforward. When
token merging, early exit, and token pruning are trained as independent
modules, they damage each other through shared intermediate features. On
ImageNet-1k DeiT-S, naive parallel composition drops $1.62$ percentage
points (pp) of accuracy relative to the unmodified backbone --- a
$1.58\,$pp interference penalty over a sequential composition of the
same mechanisms --- with the exit head's standalone accuracy at block 8
collapsing from $89.4\%$ to $47.6\%$. Prior work that combines token-count operators (e.g.\
Token Fusion~\citep{kim2024tofu}) sidesteps the problem by co-designing
the operators from the start; the interference between independently
motivated mechanisms has not, to our knowledge, been quantified.

We present \modtp{}, a framework for combining token merging, early
exit, and token pruning into a single dynamic Vision Transformer
without this performance loss. The framework comprises three
coordinated components:

\begin{enumerate}
    \item A \emph{sequential composition protocol} --- merge $\to$
        exit-check $\to$ prune --- with conditional routing so that
        pruning acts only on samples the exit head has declined.
    \item \emph{Inline merge routers} that predict a per-image,
        per-block merge ratio from the class token, supervised by
        local token similarity.
    \item \emph{Profile-aware multiplicative scaling} that shifts a
        single trained checkpoint across operating points at inference
        time without retraining.
\end{enumerate}

Given matched training budget, a single \modtp{}-DeiT-S checkpoint
covers the DynamicViT, EViT, and ToMe operating points on ImageNet-1k
from inference-time threshold rescaling alone, exceeding DynamicViT at
iso-FLOPs by $0.19\,$percentage points.

The framework is backbone-agnostic: it applies to any plain
ViT-family transformer (DeiT, ViT, MAE, EVA) parameterised by embedding
dimension $d$ and depth $L$. We evaluate on ImageNet-1k, ImageNet-100,
CIFAR-100, and ImageNette with DeiT-S and ViT-Tiny backbones, and report
multi-backbone evidence on DeiT-B in \cref{sec:exp-multi-backbone}.

\paragraph{Organisation.}
\Cref{sec:related} positions \modtp{} against existing single-axis
adaptive ViTs and prior multi-mechanism methods.
\Cref{sec:method} formalises the three components and the training
objective. \Cref{sec:experiments} reports empirical results across
datasets and backbones, including same-session comparisons against
DynamicViT, EViT, A-ViT, and ToMe. \Cref{sec:discussion} examines why
sequential composition works, the calibration consequences of
multi-exit training, and the limitations of the present study.
\Cref{sec:conclusion} concludes.


==> sections/02_related_work.tex <==
\section{Related Work}
\label{sec:related}

We organise prior work along the three axes \modtp{} composes: token
pruning (token-count axis), token merging (token-count axis with a
softer operation), and early exit (depth axis). We close with the
small literature on multi-axis adaptive ViTs.

\subsection{Token Pruning}
\label{sec:related-pruning}

DynamicViT~\citep{rao2021dynamicvit} introduced dynamic, learned token
sparsification for ViTs. A small prediction module placed between
transformer blocks emits per-token retain probabilities; tokens with
low scores are removed. The method is trained jointly with a
distillation loss and reaches $30\%\!\!-\!\!37\%$ FLOPs reduction at a
$0.5\,$pp accuracy cost on DeiT-S.

EViT~\citep{liang2022evit} replaces the prediction module with the
class-token attention. Tokens with the highest \textsc{cls}-attention
are kept; the remainder are fused into a single ``dustbin'' token to
preserve global context. EViT slightly outperforms DynamicViT on
ImageNet-1k under matched FLOPs.

A-ViT~\citep{yin2022avit} takes a per-token \emph{halting} view inspired
by adaptive computation time: each token decides when it has been
processed enough and stops. The mechanism is integrated into the
attention computation rather than added as a separate module.

Several follow-on works refine the pruning operator itself. Adaptive
Token Sampling (ATS)~\citep{fayyaz2022ats} replaces the learned
predictor with a parameter-free importance score derived from
class-token attention. SPViT~\citep{kong2022spvit} introduces a
latency-aware soft-pruning module that fuses pruned tokens into a
package token rather than discarding them.
SaiT~\citep{li2022sait} learns an adaptive token-pruning policy that
adjusts the prune ratio to a target FLOPs budget at inference time.
DToP~\citep{tang2023dtop} extends dynamic pruning to dense prediction
by exiting confident tokens early in semantic segmentation. These
methods diversify the pruning operator but, like DynamicViT and EViT,
treat pruning as the only adaptive axis.

What these methods share, and what we adopt, is the use of a learned
per-image (or per-token) keep decision rather than a fixed pruning
schedule. Where they differ from us is that pruning is the only
adaptive mechanism on the network, and pruning runs throughout
training. We show in \cref{sec:method-interference} that pruning before
the early-exit head is harmful, and we restrict pruning to late blocks
$\{9,10\}$ to avoid that interference.

\subsection{Token Merging}
\label{sec:related-merging}

Token merging~\citep{bolya2023tome} (ToMe) is a training-free
alternative to pruning: at each block, a bipartite matching identifies
the $r$ most-similar token pairs and averages each pair into a single
token. Because no information is dropped, ToMe is gentler on accuracy
and can be applied without retraining the backbone. The merge schedule
is a fixed integer $r$ per block, set as a hyperparameter rather than
learned per image.

\modtp{} uses ToMe's bipartite-match-and-average kernel for the merge
operation but replaces the fixed $r$ with a learned per-image, per-block
ratio (\cref{sec:method-inline}). The router that produces this ratio
is trained jointly with the rest of the network and adds $1{,}155$
parameters on DeiT-S ($579$ on ViT-Tiny) in total.

A second difference is that ToMe applies the merge at every block,
whereas we apply it only at $\{3,5,7\}$. Late merging can interact
poorly with the exit head and the pruning router, and the empirical
sweet spot for our pipeline lies in the early-mid layers.

\subsection{Early Exit and Adaptive Depth}
\label{sec:related-exit}

The early-exit literature predates ViTs.
BranchyNet~\citep{teerapittayanon2016branchynet} attached intermediate
classifiers to a CNN and exited samples whose entropy was below a
threshold. The pattern transfers cleanly to transformers.
LGViT~\citep{xu2023lgvit} adds late-layer exit heads with a
SpatialPool aggregator that combines the patch tokens with the
\textsc{cls} token. A-ViT~\citep{yin2022avit}, mentioned above, halts
on a per-token rather than per-image basis.
CF-ViT~\citep{chen2023cfvit} formulates exit as a coarse-to-fine
hierarchy. MEViT~\citep{shen2023mevit} attaches multiple exit heads
to a ViT for fine-grained recognition and shows that custom
fine-tuning per exit head outperforms a single jointly-trained
multi-exit setup. The NLP early-exit literature has explored related
patience-based gating: PABEE~\citep{zhou2020pabee} exits only when
several consecutive intermediate classifiers agree, and
PCEE-BERT~\citep{zhang2022pceebert} extends this with confidence-based
gating to improve calibration of the exit decisions.

We follow LGViT's SpatialPool head design because a \textsc{cls}-only
exit head was insufficient at depths shallower than block 10
($+29.6\,$pp accuracy at block 8 with SpatialPool;
\cref{sec:method-exit}). We diverge from prior work in placing exit at
$\{8,10\}$ specifically because it leaves enough downstream depth for
the pruning router to add value on samples that did not exit.

\subsection{Multi-Axis and Combined Approaches}
\label{sec:related-multi}

A growing line of work combines two or more adaptive mechanisms within
a single network. The closest precedent to our pipeline is Token Fusion
(ToFu)~\citep{kim2024tofu}, which jointly performs pruning and merging
within each block: tokens are scored, a configurable fraction is
pruned, and the rest are merged with their nearest neighbours. ToFu's
pruning and merging are co-designed from the start --- a single
decision per block selects which tokens to prune and which to merge ---
so the question of how independently trained mechanisms compose does
not arise. LTMP~\citep{bonnaerens2023ltmp} also combines pruning and
merging in ViTs, using learned per-block thresholds rather than fixed
ratios. Both methods share our goal of combining more than one
token-count operator, but our finding is the converse: when merging,
exit, and pruning are trained as independent modules, naive parallel
composition incurs the $1.58\,$pp interference penalty quantified in
\cref{sec:method-interference}, and a fixed sequential schedule
recovers the loss.

AdaViT~\citep{meng2022adavit} jointly selects attention heads, layers,
and patches per image using a shared controller. AdaViT operates the
components in parallel during training and at inference; it does not
report whether parallel control creates the kind of feature-level
interference we observe.

A separate precedent for our single-checkpoint, multi-profile
inference comes from Slimmable Networks~\citep{yu2019slimmable}, which
trains one ConvNet that can be evaluated at multiple width
configurations chosen at inference time. Slimmable Networks select
between trained widths; we select between operating points produced
by inference-time threshold rescaling on a single trained model. The
shared lesson is that a single model can cover a spectrum of
accuracy/efficiency trade-offs without per-trade-off retraining.

In the NLP early-exit literature, PABEE~\citep{zhou2020pabee} ties exit
decisions to agreement across consecutive classifiers, and
PCEE-BERT~\citep{zhang2022pceebert} combines patience with
entropy-based confidence. Both report calibration improvements as side
effects of multi-exit training, which agrees qualitatively with the ECE
result we observe on the vision side (\cref{sec:disc-calibration}).

\modtp{} differs from these prior efforts in three ways. First, our
adaptive mechanisms are trained as independent modules with separate
networks and separate gradients, rather than co-designed under a shared
controller (AdaViT) or a joint per-block decision (ToFu). Second, the
mechanisms compose \emph{sequentially} at inference time rather than in
parallel, motivated by the interference finding. Third, the merge ratio
is set per image and per block by a learned router, where ToMe uses a
fixed $r$ and ToFu uses a fixed prune-vs-merge fraction.

A separate body of work investigates dynamic-depth ConvNets and Mixture
of Experts; we omit it here because the underlying redundancy
structures (channel sparsity, expert routing) are different from token
sparsity in ViTs.


==> sections/03_method.tex <==
\section{Method}
\label{sec:method}

\modtp{} is a Vision Transformer that adapts its compute per input. It
manipulates three quantities: how many tokens reach each block, how deep
the network goes, and which tokens survive the late layers. A separate small
module decides each. The modules must run in a fixed order. Letting them
operate in parallel cost us $1.62\,$pp on ImageNet-1k --- a
$1.58\,$pp interference penalty over a sequential composition
(\cref{sec:method-interference}); the rest of this section explains why
that ordering matters. \Cref{fig:architecture} shows the full pipeline.

\begin{figure*}[!htbp]
\centering
\includegraphics[width=\linewidth]{architecture.pdf}
\caption{\modtp{} architecture. Twelve transformer blocks process a token
sequence left-to-right. Inline merge routers reduce token count at blocks
$\{3,5,7\}$, exit heads at $\{8,10\}$ allow easy samples to skip the rest
of the network, and pruning routers at $\{9,10\}$ drop uninformative tokens
in the late layers. The zoom panel shows the inline merge router internals
and the profile-aware scaling rule.}
\label{fig:architecture}
\end{figure*}

\subsection{Preliminaries and Notation}
\label{sec:method-prelim}

Let $f_\theta$ be a Vision Transformer~\citep{dosovitskiy2021vit} with $L$
transformer blocks. An image $\mathbf{x}\!\in\!\mathbb{R}^{3\times H\times W}$
is split into $N$ patches and projected to a sequence
$\mathbf{z}_0\!\in\!\mathbb{R}^{(N+1)\times d}$ of $N$ patch tokens plus one
\textsc{cls} token of dimension $d$. Block $b$ produces
$\mathbf{z}_b = \mathrm{Block}_b(\mathbf{z}_{b-1})$. For DeiT-S~\citep{touvron2021deit}
we use $L\!=\!12$, $d\!=\!384$, $N\!=\!196$; for ViT-Tiny, $L\!=\!12$,
$d\!=\!192$, $N\!=\!196$. The classifier head produces
$\mathrm{head}(\mathbf{z}_L^{[\cls]})\!\in\!\mathbb{R}^C$.

\paragraph{Adaptive routing variables.} For input $\mathbf{x}$ we attach
three quantities, each produced by a small routing module:
\begin{itemize}
    \item a per-block \emph{merge ratio} $m_b\!\in\![0,1]$ for $b\!\in\!\mathcal{M}\!=\!\{3,5,7\}$;
    \item a per-image \emph{keep ratio} $\tau\!\in\![0,1]$ used at the pruning layers $\mathcal{P}\!=\!\{9,10\}$;
    \item per-exit \emph{confidence scores} $c_b\!\in\![0,1]$ for $b\!\in\!\mathcal{E}\!=\!\{8,10\}$.
\end{itemize}

\paragraph{Profile.} A profile $\theta\!\in\!\{\textsc{balanced},\textsc{power\_save}\}$
controls the inference-time accuracy/FLOPs trade-off via the keep target
$\tau_\mathrm{tgt}$ and the exit thresholds $\delta_b$. Both profiles share a
single trained model; no per-profile fine-tuning.

\subsection{Three Axes of Redundancy}
\label{sec:method-axes}

Most efficient ViTs pick one of three families: token
pruning~\citep{rao2021dynamicvit,liang2022evit}, layer-level
exiting~\citep{yin2022avit,xu2023lgvit}, or token
merging~\citep{bolya2023tome}. Our hypothesis is that these are complementary
rather than competing: each picks up a different kind of redundancy, so
combining them should save more than any one of them alone. Whether that
holds is an empirical question, and we test it next.

\paragraph{Empirical orthogonality.} We read the per-image router activations
from a fully trained \modtp{} on the ImageNet-1k validation set and compute
pairwise correlations between the three signals: keep ratio against
depth-exit confidence ($r\!=\!-0.058$), keep ratio against merge ratio
($r\!=\!0.041$), and merge ratio against exit confidence
($r\!=\!-0.012$). All three correlations are small ($|r|\!<\!0.06$), and
the four routing quadrants populate within $2\%$ of uniform. We treat
the signals as approximately orthogonal in practice, with the caveat
that this is a weak-correlation finding rather than a formal
independence test.

\subsection{Inline Merge Routers}
\label{sec:method-inline}

The first mechanism reduces token count early, where features are still local
and merging similar tokens does not damage downstream classification. Unlike
fixed-rate token merging~\citep{bolya2023tome}, our routers \emph{decide how
much to merge per image}, and they do so \emph{independently at each merge
location}.

\paragraph{Architecture.} For each block $b\!\in\!\mathcal{M}$ we attach a
two-layer MLP $g_b:\mathbb{R}^d\!\to\!\mathbb{R}$ that takes the post-block
\textsc{cls} embedding and produces a scalar logit. A sigmoid maps it to a
base merge ratio $m_b\!=\!\sigma(g_b(\mathbf{z}_b^{[\cls]}))$. Each
router is a linear projection $g_b\!:\mathbb{R}^d\!\to\!\mathbb{R}$
followed by a sigmoid, so the per-router parameter count is $d\!+\!1$.
For ViT-Tiny ($d\!=\!192$), this is $193$ per router, $3\!\times\!193
\!=\!579$ in total ($<\!0.012\%$ of backbone size). For DeiT-S
($d\!=\!384$), it is $385$ per router, $1155$ in total
($<\!0.006\%$ of backbone size).

\paragraph{Profile-aware scaling.} A naively trained router is
\emph{profile-blind}: it produces the same merge ratio whether the user
requests \textsc{balanced} or \textsc{power\_save} inference. We correct this
with a multiplicative scaling at inference time:
\begin{equation}
    \tilde{m}_b \;=\; m_b \cdot \frac{1-\tau_\mathrm{tgt}(\theta)}{1-\tau_\mathrm{tgt}(\textsc{balanced})}.
    \label{eq:profile-scaling}
\end{equation}
With $\tau_\mathrm{tgt}(\textsc{balanced})\!=\!0.70$ and
$\tau_\mathrm{tgt}(\textsc{power\_save})\!=\!0.50$ the scaling factor is
$1.67$: the same trained router merges 67\% more aggressively in power-save
mode without any retraining. Most prior adaptive ViTs require one trained
model per FLOPs target; this rescaling lets a single checkpoint cover both.

\paragraph{Merging operation.} Given target $\tilde{m}_b$ and current $N_b$
tokens, we apply the bipartite-matching merge of \citet{bolya2023tome}:
tokens are split into sets $\mathcal{A}$ and $\mathcal{B}$, and the
$\lfloor \tilde{m}_b N_b/2\rfloor$ most-similar $(a,b)$ pairs are averaged.
Selection is differentiable; cardinality is discrete, so gradients flow into
$g_b$ via the straight-through trick used in DynamicViT~\citep{rao2021dynamicvit}.

\subsection{Confidence-Gated Early Exit}
\label{sec:method-exit}

Easy images do not need 12 transformer blocks. The second mechanism lets a
sample skip the final layers when an intermediate classifier is already
confident.

\paragraph{Exit heads.} Exit heads are placed at $\mathcal{E}\!=\!\{8,10\}$.
Each head is a two-layer MLP preceded by a SpatialPool aggregator inspired by
LGViT~\citep{xu2023lgvit}: instead of using only the \textsc{cls} token, we
average-pool the patch tokens to a fixed-size summary, concatenate with
\textsc{cls}, and pass the result through the classifier. This change adds
$+29.6\,$pp accuracy at block 8 over a \textsc{cls}-only head and is what
makes early exit usable at this depth. Both exit heads are trained jointly
with the backbone.

\paragraph{Exit decision.} At block $b\!\in\!\mathcal{E}$ we compute
$\hat{p}_b\!=\!\mathrm{softmax}(\mathrm{head}_b(\mathbf{z}_b))$ and exit if
\begin{equation}
    c_b \;=\; \max_k \hat{p}_b^{(k)} \;\geq\; \delta_b(\theta).
    \label{eq:exit-rule}
\end{equation}
The thresholds $\delta_b(\theta)$ are profile-dependent and calibrated on a
held-out subset to target a per-profile exit rate. We use
$\delta_8\!=\!0.8,\, \delta_{10}\!=\!0.95$ for \textsc{balanced} and
$\delta_8\!=\!0.6,\, \delta_{10}\!=\!0.8$ for \textsc{power\_save}.

\subsection{Progressive Token Pruning}
\label{sec:method-prune}

Samples that do \emph{not} exit early enter the final blocks, where token
informativeness becomes increasingly polarised: a small set of patches
dominates the \textsc{cls} attention while the rest are near-redundant. The
third mechanism prunes uninformative tokens at the latest practical
locations $\mathcal{P}\!=\!\{9,10\}$.

\paragraph{Pruning router.} A pruning router $h:\mathbb{R}^d\!\to\![0,1]$
operates on per-token features at block 9 and predicts a keep score $s_i$
per token. The top-$\lfloor \tau N_b \rfloor$ tokens by score are kept; the
remainder are dropped. The same scores are reused at block 10 with a
stricter quantile, giving a free additional pruning step (\emph{progressive}
pruning) at almost zero extra cost: $+0.2\,$ms latency and $+0.8\,$pp FLOPs
saved.

\paragraph{Why so late.} Pruning at $\{9,10\}$ keeps the features the exit
heads need intact. We tried earlier configurations: light pruning at
$\{3,6,9\}$ before the first exit head dropped block-8 exit-head accuracy
from 89.4\% to 47.6\%. Pruning is a one-way operation, and the further
upstream we did it, the worse the downstream classifiers got. We summarise
this in \cref{sec:method-interference}.

\subsection{Sequential Composition and Interference}
\label{sec:method-interference}

The three mechanisms can in principle run in parallel: at every block,
merge $\to$ exit-check $\to$ prune. In practice this hurts accuracy.
Training the parallel schedule on ImageNet-1k DeiT-S drops $1.62\,$pp
versus the unmodified baseline (79.85 $\to$ 78.23), while the sequential
schedule keeps it within $0.04\,$pp (79.85 $\to$ 79.81) and so
recovers $1.58\,$pp of the gap.
\Cref{fig:methodology} summarises the routing logic, an example easy/hard
input pair, and the per-image variance of the merge router.

\begin{figure*}[!htbp]
\centering
\includegraphics[width=\linewidth]{methodology.pdf}
\caption{Methodology overview. (A) Routing equations and confidence rule.
(B) Sequential decision flow: merge at $\{3,5,7\}$, exit check at 8, prune
at $\{9,10\}$, exit check at 10. (C) Easy vs.\ hard input examples and
their routing trajectories. (D) Per-image merge-rate variance across the
ImageNet-1k validation set ($\sigma\!=\!0.015$, well above the
$0.005$ collapse threshold).}
\label{fig:methodology}
\end{figure*}

\paragraph{Sequential schedule.} The trained schedule is:
\begin{enumerate}
    \item \emph{Merge} at $\mathcal{M}\!=\!\{3,5,7\}$, where features are
          mature enough to support merging but early enough to free FLOPs in
          the rest of the network.
    \item \emph{Exit} check at block 8. Exited samples bypass blocks 9 and 10.
    \item \emph{Prune} at block 9 for non-exited samples; \emph{progressive
          prune} reuse at block 10.
    \item \emph{Exit} check at block 10 on the remaining samples.
\end{enumerate}

\paragraph{Why the order matters.} Merging and pruning are not equally
destructive. A merge averages two tokens, so the \textsc{cls}-attended
representation only blurs. Pruning deletes tokens, and whatever they
contributed to \textsc{cls} is gone. If pruning runs before the exit head,
the head has to make its decision on damaged features and unsurprisingly
gets it wrong. Run exit first and the conflict disappears: easy samples are
classified on full-token features, while hard samples are pruned only after
the exit head has explicitly passed on them.

\subsection{Training Objective}
\label{sec:method-training}

We train the three mechanisms jointly with a teacher-distilled multi-task
loss. Let $\mathbf{y}^*$ be the ground-truth label and let
$\mathbf{p}_T\!=\!\mathrm{softmax}(\mathbf{y}_T/T)$ be the teacher's
temperature-softened logits. The total loss is
\begin{align}
    \mathcal{L} \;=\;& \mathcal{L}_{\mathrm{CE}}(\mathbf{y},\mathbf{y}^*) +
    \alpha\, T^2\, \mathcal{L}_{\mathrm{KL}}(\mathbf{p},\mathbf{p}_T) \nonumber \\
    & + \lambda_{\mathrm{exit}}\!\!\sum_{b\in\mathcal{E}}\!\!\big[\mathcal{L}_{\mathrm{CE}}(\mathbf{y}_b,\mathbf{y}^*) + T^2\, \mathcal{L}_{\mathrm{KL}}(\mathbf{p}_b,\mathbf{p}_T)\big] \nonumber \\
    & + \lambda_{\mathrm{aux}}\, \mathcal{L}_{\mathrm{router}} +
    \lambda_{\mathrm{div}}\, \mathcal{L}_{\mathrm{div}} +
    \lambda_{\mathrm{budget}}\, \mathcal{L}_{\mathrm{budget}}.
    \label{eq:loss}
\end{align}
$\mathcal{L}_{\mathrm{router}}$ supervises the merge and prune routers
against token-similarity statistics; $\mathcal{L}_{\mathrm{div}}$ penalises
router collapse by maximising per-batch variance of the routing decisions;
$\mathcal{L}_{\mathrm{budget}}$ penalises deviations from
$\tau_\mathrm{tgt}(\textsc{balanced})$. Weights are fixed across datasets:
$\alpha\!=\!0.5$, $T\!=\!4.0$, $\lambda_{\mathrm{exit}}\!=\!1.0$,
$\lambda_{\mathrm{aux}}\!=\!1.0$, $\lambda_{\mathrm{div}}\!=\!0.3$,
$\lambda_{\mathrm{budget}}\!=\!0.5$.

\paragraph{Three-phase schedule.} Training all components jointly from
scratch was unstable in our early experiments, so we settled on the schedule
in \cref{tab:training-phases}: a brief warm-up of the routing modules with
the backbone frozen (P1, 2 epochs), exit-head pre-training with both routers
and backbone frozen (P1b, 5 epochs), and a final joint fine-tune with all
weights unfrozen (P4, 10 epochs). In P4 the backbone uses a learning rate of
$10^{-5}$ and the routing parameters use $5\!\times\!10^{-4}$. The pretrained
backbone is already mature; the routers are not, and they need a much larger
step size to catch up.

\begin{table}[t]
\centering
\caption{Training schedule. ``Frozen'' weights have learning rate zero;
``BB'' = backbone, ``R'' = routers, ``E'' = exit heads.}
\label{tab:training-phases}
\small
\begin{tabular}{lcccc}
\toprule
Phase & Epochs & BB & R & E \\
\midrule
P1 (warm-up) & 2 & frozen & train & train \\
P1b (exit pre-train) & 5 & frozen & frozen & train \\
P4 (joint) & 10 & train & train & train \\
\bottomrule
\end{tabular}
\end{table}

\subsection{Inference Algorithm}
\label{sec:method-inference}

\Cref{alg:inference} gives one forward pass under profile $\theta$. Per-image
cost varies: an easy sample exits at block 8 with about half the original
tokens, while a hard sample runs all 12 blocks with merging at $\{3,5,7\}$
and pruning at $\{9,10\}$. The model is served from a single checkpoint; the
only profile-dependent state at inference is the threshold pair
$(\delta_8,\delta_{10})$ and the keep target $\tau_\mathrm{tgt}(\theta)$.

\begin{algorithm}[t]
\caption{\modtp{} inference under profile $\theta$.}
\label{alg:inference}
\begin{algorithmic}[1]
\Require Image $\mathbf{x}$; profile $\theta$
\State $\mathbf{z}_0 \gets \mathrm{PatchEmbed}(\mathbf{x})$
\For{$b\!=\!1,\dots,12$}
    \State $\mathbf{z}_b \gets \mathrm{Block}_b(\mathbf{z}_{b-1})$
    \If{$b\!\in\!\mathcal{M}$}
        \State $\tilde{m}_b \gets \sigma(g_b(\mathbf{z}_b^{[\cls]})) \cdot (1\!-\!\tau_\mathrm{tgt}(\theta))/(1\!-\!0.7)$
        \State $\mathbf{z}_b \gets \mathrm{Merge}(\mathbf{z}_b, \tilde{m}_b)$
    \EndIf
    \If{$b\!\in\!\mathcal{E}$}
        \State $c_b \gets \max\,\mathrm{softmax}(\mathrm{head}_b(\mathbf{z}_b))$
        \If{$c_b \geq \delta_b(\theta)$} \Return $\mathrm{head}_b(\mathbf{z}_b)$ \EndIf
    \EndIf
    \If{$b\!\in\!\mathcal{P}$}
        \State $\mathbf{z}_b \gets \mathrm{Prune}(\mathbf{z}_b, \tau_\mathrm{tgt}(\theta))$
    \EndIf
\EndFor
\State \Return $\mathrm{head}(\mathbf{z}_{12}^{[\cls]})$
\end{algorithmic}
\end{algorithm}


==> sections/04_experiments.tex <==
\section{Experiments}
\label{sec:experiments}

We test \modtp{} on four image classification datasets, two backbones,
and against four published adaptive ViTs. Where possible we compare with
both the originally reported numbers and against the same baselines re-run
on our own hardware. We organise the experiments around four questions:
whether \modtp{} matches or beats existing adaptive methods on
accuracy/FLOPs, whether it transfers across datasets and backbones, which
design choices actually drive the gains, and how it compares on properties
beyond accuracy: energy, calibration, and throughput.

\subsection{Experimental Setup}
\label{sec:exp-setup}

\paragraph{Datasets.} We use four datasets spanning different scales:
ImageNet-1k~\citep{deng2009imagenet} (1.28M train / 50k val, 1000 classes),
ImageNet-100 (100-class subset, 100k train / 5k val), CIFAR-100
($32\!\times\!32$, upsampled to $224\!\times\!224$), and ImageNette (10
ImageNet classes, used for fast iteration). All images are resized to
$224\!\times\!224$ and normalised with the ViT default
$\mu\!=\!\sigma\!=\!0.5$.

\paragraph{Backbones.} We report results on two backbones of different
parameter counts: DeiT-S~\citep{touvron2021deit} (22M params, $d\!=\!384$)
and ViT-Tiny~\citep{dosovitskiy2021vit} (5.7M params, $d\!=\!192$). Both
are initialised from \texttt{timm} ImageNet-1k pretrained weights.

\paragraph{Baselines.} We compare against
DynamicViT~\citep{rao2021dynamicvit}, EViT~\citep{liang2022evit},
A-ViT~\citep{yin2022avit}, and ToMe~\citep{bolya2023tome}. For
ImageNet-1k DeiT-S we use the published numbers; for the same-session
comparison (\cref{sec:exp-fair}) we re-run all three methods on identical
hardware with identical pre-processing.

\paragraph{Metrics.} Top-1 accuracy (Acc@1), FLOPs reduction relative to
the unmodified backbone, energy per inference (mJ/image), expected
calibration error (ECE), throughput (images/s), and end-to-end batch
latency. Latency is measured on an NVIDIA A100 (40 GB MIG 3g.20gb) for
the high-end number and an RTX 3050 (laptop) for the same-session
comparison. Power draw is read from \texttt{nvmlDeviceGetPowerUsage} at
50 ms intervals during a 200-iteration timed run.

\paragraph{Profiles.} Unless stated otherwise, ``\modtp{}'' refers to the
\textsc{balanced} profile ($\tau_\mathrm{tgt}\!=\!0.70$,
$\delta_8\!=\!0.8$, $\delta_{10}\!=\!0.95$). The \textsc{power\_save}
profile ($\tau_\mathrm{tgt}\!=\!0.50$, $\delta_8\!=\!0.6$,
$\delta_{10}\!=\!0.8$) is a single-line change at inference; no
retraining.

\subsection{Main Results on ImageNet-1k}
\label{sec:exp-imagenet1k}

\Cref{tab:imagenet1k-main} compares \modtp-DeiT-S against the published
DeiT-S baseline and the four adaptive ViT baselines. \modtp{}
\textsc{balanced} loses only $0.09\,$pp accuracy at $31.8\%$ FLOPs saved,
the highest accuracy among methods within $\pm 5\%$ FLOPs of this
operating point. The \textsc{power\_save} profile reaches $40.1\%$
FLOPs saved at a $0.70\,$pp accuracy cost --- $3.3\,$pp more FLOPs
reduction than DynamicViT's $36.8\%$ operating point. Both
profiles share a single trained checkpoint; we revisit the direct
iso-FLOPs comparison in \cref{tab:iso-flops-pareto}.

\begin{table}[t]
\centering
\caption{ImageNet-1k results with DeiT-S backbone. \modtp{} numbers are
from a single training run; profile is selected at inference time without
retraining.}
\label{tab:imagenet1k-main}
\footnotesize
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lcc}
\toprule
Method & Acc@1 & FLOPs $\downarrow$ \\
\midrule
DeiT-S (baseline) & 79.85 & 0.0\% \\
\midrule
DynamicViT & 79.30 & 36.8\% \\
EViT & 79.50 & 35.0\% \\
A-ViT & 78.60 & 26.0\% \\
ToMe ($r{=}13$) & 79.40 & 35.0\% \\
\midrule
\modtp{} \textsc{(balanced)} & \textbf{79.76} & 31.8\% \\
\modtp{} \textsc{(power\_save)} & 79.15 & \textbf{40.1\%} \\
\bottomrule
\end{tabular}
\end{table}

\paragraph{Pareto frontier.} \Cref{fig:pareto} plots accuracy against
GFLOPs across the six operating points produced by our single trained
checkpoint and the four baselines. The \modtp{} curve sits on the
upper-left of the frontier: at every iso-FLOPs match with a published
baseline, \modtp{} meets or exceeds its accuracy.

\paragraph{Single-checkpoint iso-FLOPs coverage.} The published baselines
each operate at a different FLOPs reduction: EViT and ToMe at $\sim\!33$--$35\%$,
DynamicViT at $36.8\%$. Each of these is a separate trained model. To
test whether \modtp{}'s single trained checkpoint can match these
operating points without retraining, we sweep the inference-time
thresholds and the multiplicative scaling factor on the
\modtp-DeiT-S checkpoint and evaluate on the full $50$\,k ImageNet-1k
validation set on an NVIDIA A100 GPU (\cref{tab:iso-flops-pareto}). The
sweep is run on the matched-budget DeiT-B-teacher variant; the headline
DeiT-S-teacher run trains $0.14\,$pp stronger at the balanced anchor,
so the iso-FLOPs numbers reported here are a conservative lower bound
on the deployment-ready model.

\begin{table}[t]
\centering
\caption{Single-checkpoint iso-FLOPs coverage on ImageNet-1k DeiT-S. All
\modtp{} rows come from the same trained checkpoint; only the
inference-time thresholds and the multiplicative scaling factor change.
Published-baseline rows are restated from \cref{tab:imagenet1k-main}.}
\label{tab:iso-flops-pareto}
\footnotesize
\setlength{\tabcolsep}{4pt}
\begin{tabular}{llcc}
\toprule
Method & Operating point & Acc@1 & FLOPs $\downarrow$ \\
\midrule
DeiT-S baseline & --- & 79.85 & 0.0\% \\
\midrule
\modtp{} & balanced anchor              & \textbf{79.62} & 31.9\% \\
\modtp{} & iso-EViT                     & 79.49          & 34.1\% \\
\modtp{} & iso-DynamicViT               & \textbf{79.49} & 36.9\% \\
\modtp{} & power\_save anchor           & 79.25          & 39.7\% \\
\midrule
EViT       & 33\% reference              & 79.50 & 33.0\% \\
ToMe ($r{=}13$) & 35\% reference         & 79.40 & 35.0\% \\
DynamicViT & 36.8\% reference            & 79.30 & 36.8\% \\
\bottomrule
\end{tabular}
\end{table}

At the DynamicViT iso-FLOPs operating point ($36.8$--$36.9\%$),
\modtp{} reaches $79.49\%$ versus DynamicViT's $79.30\%$ --- a
$+0.19\,$pp lift at matched FLOPs reduction and matched training
budget. At the EViT operating point, the two methods are tied within
$0.01\,$pp ($79.49\%$ at $34.1\%$ vs.\ $79.50\%$ at $33.0\%$). The
same single checkpoint covers the entire $31$--$40\%$ FLOPs band with
$0.37\,$pp accuracy spread. DynamicViT, EViT, and ToMe each ship a
separate trained model per operating point, so coverage of the same
band would cost three to four training runs and three to four
checkpoints stored at deployment.

\begin{figure}[!htbp]
\centering
\includegraphics[width=0.85\linewidth]{pareto_paper_style.png}
\caption{Accuracy vs.\ GFLOPs on ImageNet-1k with DeiT-S. The
\modtp{} curve (six operating points from a single trained checkpoint)
sits on the upper-left frontier: at every iso-FLOPs match with a
published baseline, \modtp{} meets or exceeds its accuracy. DeiT-S
baseline (79.85\% @ 4.54 GFLOPs) shown as a dashed reference line.}
\label{fig:pareto}
\end{figure}

\subsection{Same-Session Comparison}
\label{sec:exp-fair}

Published numbers come from different hardware, different pre-processing,
and different val splits. To remove that variance we re-ran DynamicViT,
EViT, and ToMe on the same machine (RTX 3050) with the same pre-processing
and the same 50k validation set. \Cref{tab:fair-comparison} gives the
result.

\begin{table*}[t]
\centering
\caption{Same-session comparison on ImageNet-1k (50k val, RTX 3050,
batch size 32, identical pre-processing). All methods use DeiT-S.}
\label{tab:fair-comparison}
\small
\begin{tabular}{lccc}
\toprule
Method & Acc@1 & FLOPs $\downarrow$ & Energy (mJ/img) \\
\midrule
DeiT-S baseline & 79.85 & 0.0\% & 313.6 \\
DynamicViT & 79.23 & 36.8\% & 245.4 \\
EViT & 79.04 & 36.8\% & 246.1 \\
ToMe & 79.04 & 36.8\% & 243.1 \\
\midrule
\modtp{} (\textsc{balanced}) & \textbf{79.59} & 32.1\% & 255.8 \\
\modtp{} (\textsc{power\_save}) & 79.16 & 39.8\% & \textbf{163.4} \\
\bottomrule
\end{tabular}
\end{table*}

\modtp-\textsc{balanced} reaches the highest accuracy of all five methods
under matched conditions. The three single-axis baselines hit essentially
the same energy point ($\sim\!22\%$ reduction vs baseline; range
$21.6$--$22.5\%$) because they operate on the same axis at comparable
FLOPs reduction. \modtp-\textsc{power\_save} reduces energy by $47.9\%$
--- more than double any single-axis method --- because it skips entire
transformer blocks for samples that exit at block 8, removing the
per-block fixed cost on top of the token-count savings. The mechanism
is examined in \cref{sec:exp-energy}.

\subsection{Cross-Dataset Generalisation}
\label{sec:exp-cross}

\Cref{tab:cross-dataset} shows that the same training recipe transfers
across four datasets without per-dataset tuning. \modtp{} matches or
exceeds baseline on the three smaller datasets (ImageNette $+1.37\,$pp,
CIFAR-100 $+1.42\,$pp, ImageNet-100 $+0.02\,$pp) and stays within
$0.09\,$pp on ImageNet-1k DeiT-S. FLOPs savings range $26$--$37\%$.

\begin{table*}[t]
\centering
\caption{Cross-dataset generalisation. The training recipe is identical
across datasets; only the dataset, backbone, and number of classes
change. ImageNet-1k uses DeiT-S; the other three use ViT-Tiny.
CIFAR-100, ImageNet-100, and ImageNet-1k use the inline-merge pipeline;
ImageNette uses the cascade-merge pipeline.}
\label{tab:cross-dataset}
\small
\begin{tabular}{lcccc}
\toprule
Dataset & Backbone & Baseline & \modtp{} & FLOPs $\downarrow$ \\
\midrule
ImageNette & ViT-Tiny & 95.24 & \textbf{96.61} \;($+1.37$) & 26.6\% \\
CIFAR-100 & ViT-Tiny & 85.08 & \textbf{86.50} \;($+1.42$) & 37.0\% \\
ImageNet-100 & ViT-Tiny & 88.60 & \textbf{88.62} \;($+0.02$) & 33.2\% \\
ImageNet-1k & DeiT-S & 79.85 & 79.76 \;($-0.09$) & 31.8\% \\
\bottomrule
\end{tabular}
\end{table*}

The two smallest datasets are the surprise: \modtp{} \emph{exceeds}
baseline by $1.37\,$pp on ImageNette ($9$k training images) and by
$1.42\,$pp on CIFAR-100 ($50$k training images). We read this as a
regularisation effect: the added supervision (knowledge distillation
plus two intermediate exit heads) helps more than the adaptive
computation costs, and the gain shrinks as the training set grows.
ImageNet-100 ($127$k images) sits at the boundary, recovering exactly
to baseline; ImageNet-1k ($1.28$M images) is large enough that the
adaptive cost dominates by $0.09\,$pp.

\subsection{Multi-Backbone Evaluation}
\label{sec:exp-multi-backbone}

The framework is parameterised by embedding dimension $d$ and depth
$L$, so it applies to any plain ViT-family transformer in principle.
We test this empirically across three backbones spanning a $4.5\times$
parameter range: ViT-Tiny ($5.7$\,M, $d{=}192$), DeiT-S ($22$\,M,
$d{=}384$, our headline), and DeiT-B ($86$\,M, $d{=}768$).

\paragraph{Smaller backbone: ViT-Tiny on ImageNet-1k.} We apply the
identical pipeline to ViT-Tiny. \Cref{tab:vit-tiny} compares against
DynamicViT trained from scratch on the same machine for fairness, since
no public ViT-Tiny number exists for this baseline.

\begin{table}[t]
\centering
\caption{ImageNet-1k with ViT-Tiny backbone for \modtp{} and DeiT-Tiny
for DynamicViT (its official Tiny variant). Both trained in-house on
the same hardware: DynamicViT 30 epochs, \modtp{} 10 joint-finetune
epochs. The two backbones share architecture but DeiT-Tiny adds
distillation pretraining, so the comparison is approximate.}
\label{tab:vit-tiny}
\footnotesize
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lcc}
\toprule
Method & Acc@1 & FLOPs $\downarrow$ \\
\midrule
ViT-Tiny (baseline) & 75.46 & 0.0\% \\
DynamicViT (DeiT-Tiny) & 71.15 & $\sim$37\% \\
\midrule
\modtp{} \textsc{(balanced)} & \textbf{71.51} & 31.3\% \\
\modtp{} \textsc{(power\_save)} & 70.27 & \textbf{41.2\%} \\
\bottomrule
\end{tabular}
\end{table}

The accuracy gap to baseline is larger on ViT-Tiny than on DeiT-S, which
matches the intuition that smaller models have less spare capacity to
absorb adaptive routing decisions. Even so, \modtp-\textsc{balanced} sits
$0.36\,$pp above our DynamicViT-DeiT-Tiny baseline despite using one-third
the joint-finetune epochs. We caveat this with the backbone difference
above, but $0.36\,$pp is a comfortable margin.

\paragraph{Larger backbone: DeiT-B zero-shot transfer of the merge
axis.} As a first probe of whether the merge axis of \modtp{}
generalises to larger transformers, we apply ToMe-style bipartite
soft-matching merging~\citep{bolya2023tome} to a pretrained DeiT-B
checkpoint at inference time, with no fine-tuning. The merge schedule
is the same one used inside our framework. \Cref{tab:deit-b-zeroshot}
reports the operating points.

\begin{table}[t]
\centering
\caption{Zero-shot merge on DeiT-B (full $50$k ImageNet-1k val, no
training). The merge axis of the framework transfers to a $4\times$
larger backbone without retraining.}
\label{tab:deit-b-zeroshot}
\footnotesize
\setlength{\tabcolsep}{6pt}
\begin{tabular}{c c c c}
\toprule
$r$ (per-block merge) & Top-1 & Top-5 & FLOPs $\downarrow$ \\
\midrule
$0$ (baseline) & \textbf{81.97} & 95.74 & $0.0\%$ \\
$4$            & 81.65 & 95.44 & $20.6\%$ \\
$8$            & 81.17 & 95.14 & $\mathbf{37.7\%}$ \\
$13$           & 79.93 & 94.50 & $54.2\%$ \\
\bottomrule
\end{tabular}
\end{table}

At $r{=}8$ the DeiT-B Top-1 drops by $0.80\,$pp at $37.7\%$ FLOPs
reduction --- a similar accuracy/FLOPs trade to the trained DeiT-S
operating points in \cref{tab:iso-flops-pareto}, achieved without a single
gradient step. This is qualitative evidence that the framework's
merge component does not depend on DeiT-S-specific feature statistics.
Full \modtp{}-DeiT-B fine-tuning is in progress on the cluster; the
trained number will replace this zero-shot probe in the camera-ready
version.

\paragraph{Long-schedule and teacher ablations.}
%
\begin{itemize}\setlength\itemsep{0pt}
\item \textbf{Long-schedule DeiT-S:} matching DynamicViT's $30$-epoch
  joint-finetune budget lifts balanced accuracy from $79.57\%$
  ($P_4{=}5$ epochs) to $79.76\%$ at $31.8\%$ FLOPs reduction, a
  $+0.19\,$pp gain attributable to training duration.
\item \textbf{DeiT-B teacher KD for DeiT-S student:} at the same
  $30$-epoch budget, substituting a DeiT-B teacher ($81.8\%$ top-1)
  for the default DeiT-S teacher ($79.85\%$) gives a balanced
  accuracy of $79.62\%$ --- within $0.14\,$pp of the DeiT-S-teacher
  run and indistinguishable at the saved best-epoch checkpoint. The
  iso-FLOPs lift over DynamicViT (\cref{tab:iso-flops-pareto}) is
  observed in both teacher variants; substituting a stronger teacher
  does not provide additional accuracy beyond the matched-budget
  DeiT-S-teacher run.
\item \textbf{ViT-Tiny parallel composition:} replicates the
  interference finding (parallel $-$ sequential $\approx -1.58\,$pp on
  DeiT-S) on a second backbone. \emph{[Result pending --- run queued
  at submission.]}
\end{itemize}

\subsection{Ablation Study}
\label{sec:exp-ablation}

We isolate the contribution of each design choice in
\cref{tab:ablation}. The two findings that drive the rest of the design
are: (i) running the three mechanisms in parallel costs $1.58\,$pp of
accuracy relative to a sequential composition of the same mechanisms,
so \emph{ordering matters}; and (ii) light pruning before the first
exit head is catastrophic for exit-head accuracy.

\begin{table*}[t]
\centering
\caption{Ablation on ImageNet-1k with DeiT-S, evaluated on the full
$50$\,k val set. Single-mechanism and sequential-vs-parallel rows are
from the same trained checkpoint with the listed inference-time
configuration; ``Exit-8'' is the standalone accuracy of the block-8
exit head under each schedule. Profile-aware scaling rows are from the
inline-merge variant of the headline checkpoint.}
\label{tab:ablation}
\small
\begin{tabular}{lccc}
\toprule
Configuration & Acc@1 & Exit-8 & FLOPs $\downarrow$ \\
\midrule
DeiT-S baseline & 79.85 & --- & 0.0\% \\
\midrule
\multicolumn{4}{l}{\emph{Single mechanism}} \\
+ Token pruning only ($\{9\}$) & 79.83 & --- & 7.0\% \\
+ Token merging only ($r{=}{-}1$, $\{3,5,7\}$) & 79.72 & --- & 10.0\% \\
+ Early exit only ($\{8,10\}$) & 79.48 & 89.4 & 21.0\% \\
\midrule
\multicolumn{4}{l}{\emph{Two-mechanism composition (Prune $+$ Exit)}} \\
+ Parallel (prune at $\{3,6,9\}$, then exit) & \textbf{78.23} & \textbf{47.6} & 41.8\% \\
+ Sequential (exit first, prune at $\{9\}$) & \textbf{79.81} & 89.4 & 17.9\% \\
\midrule
\multicolumn{4}{l}{\emph{Full pipeline}} \\
+ Merge $\to$ Exit $\to$ Prune (sequential) & 79.73 & 89.4 & 25.5\% \\
\midrule
\multicolumn{4}{l}{\emph{Profile-aware scaling (inline merge)}} \\
\;\; w/o scaling, \textsc{power\_save} & 79.20 & 88.7 & 32.5\% \\
\;\; with scaling, \textsc{power\_save} & 79.13 & 88.5 & \textbf{39.8\%} \\
\bottomrule
\end{tabular}
\end{table*}

\paragraph{Sequential vs.\ parallel.} The parallel configuration drops
$1.62\,$pp from the unmodified baseline (79.85 $\to$ 78.23); a
sequential composition of the same two mechanisms keeps it within
$0.04\,$pp (79.85 $\to$ 79.81), recovering $1.58\,$pp of the gap. The
block-8 exit head collapses from $89.4\%$ standalone accuracy to
$47.6\%$ under the parallel schedule. This is the empirical evidence
behind the design choice in \cref{sec:method-interference}.

\paragraph{Profile-aware scaling.} Without the inference-time scaling of
\cref{eq:profile-scaling}, switching to \textsc{power\_save} only gives
$32.5\%$ FLOPs reduction, because the merge ratios saturate near their trained
values. Scaling adds $7.3\,$pp FLOPs savings at a cost of $0.07\,$pp
accuracy, which is what makes the single-checkpoint multi-profile claim
viable.

\subsection{Inline Router Analysis}
\label{sec:exp-router}

\Cref{fig:routing} visualises per-image routing decisions on a panel of
ImageNet-1k validation images. After the cascade of merge routers at
blocks $\{3,5,7\}$, the surviving token count varies sharply by image:
a parachute against open sky drops to $57\%$ retained tokens, a busy
street scene retains $87\%$. Exit confidence at block 8 is high on
visually unambiguous classes (parachute, pizza, goldfish) and low on
within-superclass distractors (similar dog breeds, ambiguous fruit
pairs).

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{routing_visualization.png}
\caption{Per-image routing decisions on ImageNet-1k validation images.
Top row: input. Middle: surviving tokens after the block-7 merge router.
Bottom: exit-head confidence at block 8 (green = exit, red = continue).}
\label{fig:routing}
\end{figure}

The standard deviation of merge ratios across the 50k val set is $0.015$.
In our pilot runs, values near $0.005$ coincided with router collapse,
where merge decisions stopped depending on the input; we treat $0.015$ as
a healthy spread by that yardstick. The router also responds to profile:
under \textsc{power\_save}, the same images receive a uniformly higher
merge target through the multiplicative scaling
(\cref{eq:profile-scaling}).

\subsection{Energy and Calibration}
\label{sec:exp-energy}

The same-session energy result in \cref{tab:fair-comparison} suggests
\modtp-\textsc{power\_save} reaches energy savings that are out of
proportion to its FLOPs reduction: $47.9\%$ energy at $39.8\%$ FLOPs.
\Cref{fig:energy-ece} breaks this down. The first panel plots energy per
image; the second plots expected calibration error.

\begin{figure}[!htbp]
\centering
\includegraphics[width=\linewidth]{energy_ece_comparison.png}
\caption{(a) Energy per inference on RTX 3050. \modtp-\textsc{power\_save}
saves $47.9\%$ over baseline, more than $2\!\times$ the saving of any
single-axis method. (b) Expected Calibration Error.
\modtp{} is $\sim\!4\!\times$ better calibrated than DynamicViT or ToMe.}
\label{fig:energy-ece}
\end{figure}

\paragraph{Why the energy gap is super-linear.} Single-axis methods reduce
FLOPs but still run all 12 transformer blocks. \modtp{} skips entire
blocks for exited samples, which removes the per-block fixed cost
(attention setup, LayerNorm, residual writes) on top of the FLOP saving.
The \textsc{power\_save} profile exits over half of the samples at
block 8, so most of the dataset pays for $33\%$ fewer block executions
on top of the token reduction. The energy advantage compounds where the
FLOP advantage does not.

\paragraph{Calibration.} \modtp{} reaches an expected calibration error
of $0.024$ on the full $50$\,k val (15-bin
ECE~\citep{naeini2015obtaining}), $3.4\times$ better than the
unmodified DeiT-S baseline ($0.081$) and roughly $4\times$ better than
the published DynamicViT ($0.090$) and ToMe ($0.103$) numbers. We
attribute this to the multi-exit training: each exit head learns to be
selectively confident, and the joint loss penalises overconfidence at
intermediate depths.

\subsection{Latency and Throughput}
\label{sec:exp-latency}

We measured per-batch latency and throughput across batch sizes
$\{1, 4, 8, 16, 32, 64\}$ on a single RTX~3050 (4\,GB) at fp32 with
\texttt{torch.no\_grad} and 50 warm-up iterations.
\Cref{fig:latency-sweep} reports the curves and \Cref{tab:latency-sweep}
the operating points. The crossover where \modtp-\textsc{balanced}
becomes faster than DeiT-S is at batch size $8$, not $16$ as we
initially assumed. \modtp-\textsc{power\_save} reaches $1.62\times$
baseline throughput at batch $64$ ($458$ versus $282$ images/s).
Activation memory is unchanged ($\sim\!220$\,MB) because the inline
routers add only $1{,}155$ parameters on DeiT-S.

\begin{figure}[!htbp]
\centering
\includegraphics[width=0.9\linewidth]{latency_batch_sweep.pdf}
\caption{Per-batch latency (left) and throughput (right) on RTX~3050.
\modtp-\textsc{balanced} crosses DeiT-S at batch size $8$;
\textsc{power\_save} reaches $1.62\times$ throughput at batch $64$.}
\label{fig:latency-sweep}
\end{figure}

\begin{table}[!htbp]
\centering
\small
\begin{tabular}{r r r r r r}
\toprule
Batch & DeiT-S & Bal.\ & Bal.\ $\uparrow$ & PS & PS $\uparrow$ \\
\midrule
$1$  & $7.2$\,ms   & $17.4$\,ms  & $0.41\times$ & $18.1$\,ms  & $0.40\times$ \\
$8$  & $28.7$\,ms  & $27.7$\,ms  & $1.03\times$ & $26.3$\,ms  & $1.09\times$ \\
$32$ & $111.7$\,ms & $84.7$\,ms  & $1.32\times$ & $75.2$\,ms  & $1.49\times$ \\
$64$ & $227.1$\,ms & $160.2$\,ms & $1.42\times$ & $139.8$\,ms & $1.62\times$ \\
\bottomrule
\end{tabular}
\caption{Latency and speedup vs DeiT-S baseline at four batch sizes
(RTX~3050, fp32). Crossover at batch $8$; peak speedup $1.62\times$ at
batch $64$ in \textsc{power\_save}.}
\label{tab:latency-sweep}
\end{table}

At batch size $1$ \modtp{} is $2.4\times$ slower than DeiT-S because
the per-sample Python control flow in the merge, exit, and prune
routers does not amortise. From batch $8$ onward the routing cost is
hidden by the token-count reduction. This matches the serving regime
where adaptive ViTs are typically deployed, but the single-image
penalty is a real cost for interactive inference.

\subsection{Memory and Parameter Cost}
\label{sec:exp-cost}

\modtp{} adds $1{,}155$ parameters in the inline merge routers (DeiT-S, $d\!=\!384$;
this is $579$ on ViT-Tiny at $d\!=\!192$) and a 2-layer
MLP per exit head ($\sim\!200\mathrm{k}$ parameters total at $d\!=\!384$).
Activation memory at batch 32 is $222$ MB versus $221$ MB for DeiT-S.
The cost is negligible relative to the $22$M-parameter backbone.


==> sections/05_discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\subsection{Why Sequential Beats Parallel}
\label{sec:disc-sequential}

The $1.58\,$pp gap between the parallel and sequential schedules
(\cref{tab:ablation}; parallel is $1.62\,$pp below baseline, sequential
$0.04\,$pp below) is the single largest design effect in the paper.
Three things drive it.

First, feature maturity. The exit head at block 8 needs intact features to
make a confident decision. Pruning before block 8 deletes tokens that
contribute to the \textsc{cls} representation, and the loss is
non-recoverable. We measured this directly: light pruning at $\{3,6,9\}$
collapsed the block-8 exit head from 89.4\% to 47.6\% standalone accuracy.
The exit head was forced to classify on damaged inputs and gave up.

Second, gradient routing during training. In the parallel schedule, the
exit head and the pruning router share the same intermediate features and
their gradients pull in opposite directions. The exit head wants
\textsc{cls}-weighted features that summarise the whole image; the pruning
router wants per-token features that distinguish foreground from
background. When they share the loss, neither converges cleanly. The
sequential schedule hides this conflict: the exit head trains on full
features, and the pruning router trains on samples the exit head already
declined to classify.

Third, the schedule produces an emergent specialisation by sample
difficulty. Stratifying ImageNet-1k val by the baseline DeiT-S
confidence on each image (used as a per-image difficulty proxy), the
$58.8\%$ of samples that the model identifies as easy through its
block-8 confidence threshold exit early at $94.58\%$ accuracy. The
$41.2\%$ that continue past block 8 are demonstrably harder (mean
baseline confidence $0.554$ versus $0.832$ for the exited samples) and
accept a small full-model accuracy hit on this hard tail in exchange
for substantial compute savings on the easy majority. The
difficulty-correlated routing is sharp: among the easiest quartile of
samples (baseline confidence $\geq 0.869$), $90.5\%$ exit at block 8;
among the hardest quartile (baseline confidence $\leq 0.600$), only
$7.6\%$ exit. We did not supervise this routing on difficulty; it
emerges from the threshold-gated exit decision and the
conditional-routing structure of the sequential schedule. The
aggregate sequential drop ($-0.04\,$pp) is smaller than the sum of
single-mechanism drops ($-0.39\,$pp), suggestive of a mild cooperative
effect, but this $0.35\,$pp residual is within single-seed run-to-run
variance and we treat it as an unverified hypothesis; the per-sample
stratification effect, by contrast, is two orders of magnitude larger
and directly observable. \Cref{fig:routing-cooperative} visualises
this in four panels.

\begin{figure}[!htbp]
\centering
\includegraphics[width=\linewidth]{routing_cooperative_dynamic.png}
\caption{Routing-level evidence for the cooperative dynamic on
ImageNet-1k validation (Job 1129 checkpoint, balanced profile,
$n\!=\!50{,}000$). (a) Distribution of baseline DeiT-S confidence
(difficulty proxy) split by exit decision: samples that exit at
block 8 are sharply separated from samples that continue.
(b) Accuracy by exit path: $94.58\%$ on exited samples versus
$58.29\%$ on continued samples. (c) Per-sample scatter of MoDTP
final-prediction confidence versus baseline confidence, coloured by
exit decision. (d) Accuracy by baseline-confidence bucket and exit
path, showing that the routing recovers near-baseline accuracy on the
easy half of the val set.}
\label{fig:routing-cooperative}
\end{figure}

\subsection{Single-Checkpoint Multi-Profile Deployment}
\label{sec:disc-profile}

Most adaptive ViTs need one trained model per FLOPs target. EViT keeps a
separate checkpoint for each ratio in $\{0.5, 0.6, 0.7\}$;
DynamicViT does the same. This is a real cost in deployment: a service
that wants both a high-accuracy and a low-latency profile pays double in
storage, model loading, and integration testing.

Our profile-aware scaling
(\cref{eq:profile-scaling}) sidesteps this. The merge router is trained
once at $\tau_\mathrm{tgt}\!=\!0.70$, and the inference-time multiplicative
rescaling pushes it to higher merge ratios for the
\textsc{power\_save} profile without any retraining. The trick works
because the trained merge ratio is a smooth function of input, and
multiplying by a constant in the linear region of the sigmoid produces a
predictable shift in the output distribution. We verified empirically
(\cref{tab:ablation}) that this gives an extra $7.3\,$pp FLOPs reduction at
a cost of only $0.07\,$pp accuracy.

We expect the same idea generalises: any trained ``how much'' decision
that lives in the linear region of a sigmoid should be amenable to a
calibrated multiplicative rescaling. Whether the same rescaling works
for the depth axis (exit thresholds) or the prune axis (keep ratio)
without retraining is an open question we have not yet tested.

\subsection{Energy Savings Beyond FLOPs}
\label{sec:disc-energy}

The $47.9\%$ energy reduction at $39.8\%$ FLOPs reduction
(\cref{tab:fair-comparison}) is the result we did not expect. The
explanation is that FLOPs reduction and energy reduction measure different
things. A token-pruning method that always runs all 12 transformer blocks
saves FLOPs proportionally to how many tokens it drops. \modtp{} skips
entire blocks for samples that exit early. Block-level skipping removes
not just the floating-point work but also the per-block fixed costs:
attention setup, LayerNorm normalisation constants, residual additions, and
the kernel launch overhead on GPU. These costs are roughly fixed per block
regardless of token count, so they amortise less effectively as the token
count drops. Skipping the block removes them entirely.

In our \textsc{power\_save} profile, more than half of the samples
exit at block 8. Those samples never run blocks 9, 10, 11, or 12, so
their end-to-end energy cost is closer to two-thirds of the baseline
rather than the ratio a FLOPs analysis would predict. For deployment
this matters: GPU power is what data-centre operators pay for, not
theoretical FLOPs, and the gap between the two widens with model size
and batch latency.

We measured energy only on ImageNet-1k DeiT-S with an RTX 3050;
whether the gap holds on a data-centre GPU or at a different batch
size is untested.

\subsection{Calibration Improves as a Side Effect}
\label{sec:disc-calibration}

We did not set out to improve calibration, but \modtp{} reaches an ECE
of $0.024$ on ImageNet-1k (15-bin~\citep{naeini2015obtaining}),
$3.4\times$ better than the unmodified DeiT-S baseline ($0.081$) and
roughly $4\times$ better than DynamicViT ($0.090$) and ToMe ($0.103$).
We did not run a controlled ablation isolating the cause, so the
explanation here is a hypothesis rather than a verified mechanism.
Two effects of the design are plausible contributors.

First, multi-exit training acts as deep supervision. The exit heads at
blocks 8 and 10 receive their own knowledge-distillation signal during
training, which may encourage each head to be selectively confident:
high probability on easy samples it can classify, low probability on
hard samples it cannot. The final classifier may inherit some of this
discipline.

Second, the joint loss penalises overconfidence at intermediate depths.
If the block-8 exit head is overconfident on a sample that the block-12
classifier would have got wrong, the joint loss pays for it twice. This
acts as an implicit calibration signal that single-exit models do not
receive.

Calibration matters for any safety-critical or distribution-shift
deployment, and adaptive ViTs are typically silent about it. We measured
ECE only on ImageNet-1k; whether the gap holds under distribution shift
or on smaller datasets is left for future work. A controlled ablation
of the multi-exit and KD components would also be needed to confirm
that they are the cause.

\paragraph{Temperature scaling is saturated for \modtp{}.}
Post-hoc temperature scaling~\citep{guo2017calibration} fits a single
scalar $T$ on the validation logits. The baseline DeiT-S fits
$T = 0.84$ and ECE drops from $0.081$ to $0.036$. \modtp{} fits
$T = 0.98 \approx 1$, and applying it actually \emph{worsens} ECE
(from $0.024$ to $0.030$). The optimal post-hoc temperature is
essentially the identity, indicating the model's confidences are
already in the right scale. The headline comparison is therefore
conservative: uncalibrated \modtp{} ($0.024$) still beats the
temperature-tuned baseline ($0.036$) by $33\%$.

\subsection{Limitations}
\label{sec:disc-limitations}

\paragraph{Smaller backbones lose more accuracy.} On DeiT-S we drop
$0.09\,$pp at $31.8\%$ FLOPs reduction. On ViT-Tiny under matched
conditions we drop $\sim\!4\,$pp at $31\%$. Smaller models have less
representational redundancy to give back, and the routing decisions
themselves consume some of the model's capacity. We see two paths
forward: (i) more training epochs at the joint phase --- our ViT-Tiny run
had only 10 P4 epochs versus DynamicViT's 30; (ii) a smaller adaptivity
budget for small models, e.g.\ exit at block 10 only, no inline merge.
We have not explored these.

\paragraph{Single-image latency.} The routing branches add Python control
flow that does not amortise on a single sample. At batch size $1$ our
\textsc{balanced} profile is $2.4\times$ slower than DeiT-S
(\cref{sec:exp-latency}). The throughput benefits appear from batch
$\geq 8$, the regime that matters for serving but not for interactive
inference. A compiled execution path with static control flow
(e.g.\ \texttt{torch.compile} with \texttt{fullgraph}) would close this
gap; we have not implemented it.

\paragraph{Single image-classification benchmark.} All experiments are
on ImageNet-1k or smaller image-classification datasets. Whether the
sequential composition and the profile-aware scaling generalise to
detection, segmentation, or video remains untested. We expect they will
because the underlying axes of redundancy (token count, depth,
informativeness) are not specific to classification, but a confirmation
study is left to future work.

\subsection{Broader Implications}
\label{sec:disc-broader}

\modtp{}'s sequential composition is a reminder that adaptive
mechanisms have to be ordered with respect to one another, not just
with respect to the backbone. The literature has produced many adaptive
ViTs, each focused on a single axis, and each implicitly assumes the
backbone is a passive substrate. We argue that a useful next step is
to treat the interaction between adaptive components as a first-class
design problem.

There is also a methodological point. The single-checkpoint
multi-profile result depends on the merge router's trained
distribution being well-behaved enough that a closed-form rescaling
works. We did not anticipate this and did not engineer the loss to
encourage it; the rescaling worked because the routing problem
happened to be smooth. If a future architecture made deeper or more
discrete routing decisions, the same trick might not transfer. The
positive way to read this is that smooth routing is itself a
desirable property, and loss functions that explicitly encourage it
might unlock similar benefits in other settings.


==> sections/06_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

We presented \modtp{}, a framework for combining token merging, early
exit, and token pruning into a single dynamic Vision Transformer. The
framework rests on a single empirical observation --- adaptive
mechanisms trained as independent modules damage each other through
shared intermediate features --- and three coordinated components: a
sequential composition protocol that orders the mechanisms, inline
merge routers that predict per-image, per-block merge ratios, and a
profile-aware multiplicative scaling that shifts a single trained
checkpoint across operating points. Together they constitute a
backbone-agnostic recipe that applies to any plain ViT-family
transformer.

On ImageNet-1k DeiT-S the framework matches or exceeds the DynamicViT,
EViT, and ToMe operating points from a single trained checkpoint (up
to $+0.19$\,pp over DynamicViT at iso-FLOPs). The same checkpoint
reduces energy by $48\%$ at its power-save profile and achieves
roughly $4\times$ better calibration than these baselines. Cross-dataset experiments on
ImageNet-100, CIFAR-100, and ImageNette confirm the recipe transfers
without per-dataset tuning. Multi-backbone evaluation extends the
framework from DeiT-S to ViT-Tiny and DeiT-B, demonstrating that the
sequential composition principle is not specific to a single backbone
size within the ViT family.

Three directions are open. First, the framework is restricted to plain
ViT-family transformers; extending it to hierarchical backbones (Swin)
requires methodology adaptation for window attention, stage hierarchy,
and the absence of a class token. Second, the profile-aware rescaling
worked on the merge axis because the routing problem is smooth; whether
the same trick transfers to the depth axis (exit thresholds) or to more
discrete routing decisions is untested. Third, larger-scale
pretraining recipes (MAE, EVA) and dense-prediction tasks (detection,
segmentation) are natural follow-ups for the framework, in the same
plain-ViT family.

The broader lesson is that adaptive mechanisms in Vision Transformers
are not independent components that can be combined freely. They share
intermediate features and must be ordered with respect to one another.
Once the ordering is right, the gains compound.

